AbRank: A Benchmark Dataset and Metric-Learning Framework for Antibody-Antigen Affinity Ranking

Accurate prediction of antibody-antigen (Ab-Ag) binding affinity is essential for therapeutic design and vaccine development, yet the performance of current models is limited by noisy experimental labels, heterogeneous assay conditions, and poor generalization across the vast antibody and antigen sequence space. We introduce AbRank, a large-scale benchmark and evaluation framework that reframes affinity prediction as a pairwise ranking problem. AbRank aggregates over 380,000 binding assays from nine heterogeneous sources, spanning diverse antibodies, antigens, and experimental conditions, and introduces standardized data splits that systematically increase distribution shift, from local perturbations such as point mutations to broad generalization across novel antigens and antibodies. To ensure robust supervision, AbRank defines an m-confident ranking framework by filtering out comparisons with marginal affinity differences, focusing training on pairs with at least an m-fold difference in measured binding strength. As a baseline for the benchmark, we introduce WALLE-Affinity, a graph-based approach that integrates protein language model embeddings with structural information to predict pairwise binding preferences. Our benchmarks reveal significant limitations in current methods under realistic generalization settings and demonstrate that ranking-based training improves robustness and transferability. In summary, AbRank offers a robust foundation for machine learning models to generalize across the antibody-antigen space, with direct relevance for scalable, structure-aware antibody therapeutic design.

==> chapters/SI.tex <==
\section*{Supplementary Materials}

\subsection*{Dataset Documentation and Intended Uses}

==> chapters/acknowledgements.tex <==
\section{Acknowledgments}
% CL was part-funded by a UCL Centre for Digital Innovation Amazon Web Services (AWS) Scholarship; LD was funded by an ISMB MRC iCASE Studentship (MR/R015759/1).
% We would also like to thank the NeurIPS reviewers for their valuable feedback and suggestions, which helped us improve the clarity and quality of this work.


==> chapters/archive/Checklist.tex <==
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}{\bf Limitations are discussed in the paper, although there is no separate section.  See \cref{sec:WALLE_graph-based_method} where the limitations of our graph-based method are discussed, such as its performance degeneration when using epitope-group data splitting, and bias toward seen epitopes. The imbalance of epitope types in the AsEP dataset is also discussed. Furthermore, the limitation to conventional antibodies is made clear (\cref{sec:WALLE_graph-based_method}). 
    Assumptions made, for example, regarding distance cut-offs for epitope definition or prediction thresholds, are either based on established conventions from previous works or optimized for empirically.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}{\bf In an impact statement in \cref{sec:appendix-impact-statement} we discuss potential negative impacts of our work. However, this is minimal as it does not directly apply to this field.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}{\bf In the abstract section, we provide the link to the GitHub repository with instructions to reproduce our experiments and download the dataset.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}{\bf \cref{sec:appendix-build-abag-dataset}: steps to build the dataset; \cref{sec:dataset-split}: dataset split; \cref{sec:appendix-implementation-details}: hyperparameters and tunning; \cref{sec:hparam-tuning}: details of hyperparameter tuning}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}{\bf \cref{tab:benchmark-performance} provided standard errors}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}{\bf These are provided in~\cref{sec:appendix-implementation-details}}
\end{enumerate}1304923


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}{\bf All methods are cited in section~\cref{sec:PreviousWork}.}
  \item Did you mention the license of the assets?
    \answerYes{}{\bf The license of the data set, Creative Commons Attribution 4.0 International, is provided in the data online storage at Zenodo with DOI: \texttt{10.5281/zenodo.11495514}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}{\bf In the abstract, we provide the link to the GitHub repository with instructions to reproduce our experiments and download the dataset.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{}{\bf The original source of the dataset is derived from Protein Data Bank with a CC0 1.0 UNIVERSAL license}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}{\bf The presented dataset does not contain any personally identifiable information or offensive content}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> chapters/archive/SI.tex <==
\section*{Supplementary Materials}

\subsection*{Dataset Documentation and Intended Uses}

We provide a data card for this dataset, \texttt{DataCard-AsEP.md}, which can be downloaded using this link: \url{https://drive.google.com/file/d/1fc5kFcmUdKhyt3WmS30oLLPgnkyEeUjJ/view?usp=drive_link}

This dataset provides a unified benchmark for researchers to develop new machine-learning-based methods for the epitope prediction task.

\subsection*{Access to the Dataset}

There are two alternative sources where users can download the dataset:

\begin{itemize}
    \item The dataset can be downloaded using the Python interface provided by our GitHub Repository \href{https://github.com/biochunan/AsEP-dataset}{AsEP-dataset}. Detailed instructions on how to download the dataset are provided in the README file. Briefly, after installing the provided Python module, \texttt{asep}, the dataset can be downloaded by running the following command in the terminal:
    % \begin{lstlisting}[language=bash]
    \begin{minted}{bash}
    download-asep /path/to/directory AsEP
    # For example, to download the dataset to the current directory, run
    # download-asep . AsEP
    \end{minted}
    \item The dataset and benchmark are provided through Zenodo at \url{https://doi.org/10.5281/zenodo.11495514}.
    \item Code and Dataset interface is provided in our GitHub Repository \textbf{AsEP-dataset} at \url{https://github.com/biochunan/AsEP-dataset}.
\end{itemize}

\subsection*{Author Statement}

The authors affirm that they bear all responsibility in case of violation of rights, etc., and confirm the data license. 
The dataset is licensed under the \textbf{CC BY 4.0} License (\url{https://creativecommons.org/licenses/by/4.0/}), which is provided through the Zenodo repository. 
The code is licensed under the \textbf{MIT License} (\url{https://opensource.org/licenses/MIT}).

\subsection*{Hosting, Licensing, and Maintenance Plan}
The dataset is hosted on Zenodo, which provides a DOI (10.5281/zenodo.11495514) for the dataset. 
It also comes with a Python interface provided in our GitHub Repository, AsEP-dataset at \url{https://github.com/biochunan/AsEP-dataset}, where users can submit issues and ask questions. 
Future releases and updates will be made available through the same channels. 
As discussed in the main text, the future plan includes expanding the dataset to include novel types of antibodies, such as single-domain antibodies, and providing more sophisticated features for graph representations. 
The dataset will be maintained by the authors and will be available for a long time.

\subsection*{Links to Access the Dataset and Its Metadata}
The dataset, benchmark, and metadata are provided through \href{https://doi.org/10.5281/zenodo.11495514}{Zenodo}.

\subsection*{The Dataset}

The dataset is constructed using \texttt{pytorch-geometric Dataset} module. The dataset can be loaded using the following code:

\begin{minted}{python}
from asep.data.asepv1_dataset import AsEPv1Evaluator

evaluator = AsEPv1Evaluator()

# example
torch.manual_seed(0)
y_pred = torch.rand(1000)
y_true = torch.randint(0, 2, (1000,))

input_dict = {'y_pred': y_pred, 'y_true': y_true}
result_dict = evaluator.eval(input_dict)
print(result_dict)  # got {'auc-prc': tensor(0.5565)}
% \end{lstlisting}
\end{minted}

We also provide detailed documentation of the dataset content on Zenodo and include a description below:

\begin{itemize}
  \item \texttt{asepv1-AbDb-IDs.txt}: A text file containing the AbDb identifiers of the 1723 antibody-antigen pairs in the dataset.
  \item \texttt{asepv1\_interim\_graphs.tar.gz}: Contains 1723 \texttt{.pt} files, where each file is a dictionary with structured data:
  \begin{description}
    \item[\texttt{abdbid}] A string representing the antibody AbDb identifier.
    \item[\texttt{seqres}] A dictionary containing:
    \begin{description}
      \item[\texttt{ab}] An OrderedDict mapping string chain labels \texttt{H} and \texttt{L} to their corresponding sequence strings, representing heavy and light chains respectively.
      \item[\texttt{ag}] A dictionary mapping string chain labels to their corresponding sequence strings.
    \end{description}
    \item[\texttt{mapping}] Includes:
    \begin{description}
      \item[\texttt{ab}] Contains:
      \begin{description}
        \item[\texttt{seqres2cdr}] A binary numpy array indicating the CDR positions in the antibody sequence.
      \end{description}
      \item[\texttt{ag}] Contains:
      \begin{description}
        \item[\texttt{seqres2surf}] A binary numpy array indicating the surface residues in the antigen sequence.
        \item[\texttt{seqres2epitope}] A binary numpy array indicating the epitope residues in the antigen sequence.
      \end{description}
    \end{description}
    \item[\texttt{embedding}] Comprises:
    \begin{description}
      \item[\texttt{ab}] Includes embeddings computed using the AntiBERTy model and ESM2 model for the antibody sequences.
      \item[\texttt{ag}] Includes embeddings for the antigen sequences computed using the ESM2 model.
    \end{description}
    \item[\texttt{edges}] Describes the interactions:
    \begin{description}
      \item[\texttt{ab}] A sparse coo tensor representing the binary edges between the CDR residues.
      \item[\texttt{ag}] A sparse coo tensor representing the binary edges between the surface residues.
    \end{description}
    \item[\texttt{stats}] Metadata about each antibody-antigen pair, including counts of CDR, surface, and epitope residues, and the epitope-to-surface ratio.
  \end{description}
  \item \texttt{structures.tar.gz}: Contains \texttt{1723} pdb structures, each named using the AbDb identifier.
  \item \texttt{split\_dict.pt}: Contains the \texttt{train}/\texttt{val}/\texttt{test} splits of the dataset, with splits based on the epitope ratio and epitope group of the antigen.
\end{itemize}

\subsection*{Long-term Preservation}

The current version of the dataset and benchmark are provided through Zenodo, which provides long-term storage. 
Future versions will be made available through the same channel and users are encouraged to submit queries and issues through the issues channel on the GitHub repository.

\subsection*{Explicit License}

The dataset is licensed under the \textbf{CC BY 4.0} license (\url{https://creativecommons.org/licenses/by/4.0/}), which is provided through the Zenodo repository. 
The code is licensed under the MIT License \url{https://opensource.org/licenses/MIT}.

\subsection*{Benchmarks}

Detailed benchmark experiments and results are provided on Zenodo (\url{https://doi.org/10.5281/zenodo.11495514}), and the file \texttt{benchmark.zip} contains the instructions on how to reproduce the results. 
To run ESMFold, EpiPred, and MaSIF-Site, we provided docker images on the Zenodo repository or instructions on how to obtain them from DockerHub. 
The benchmark results are reproducible by following the instructions provided in the zip file. 
For the method WALLE and its variants used in the ablation studies, their configuration YAML files and the trained models are also provided on Zenodo.

